Neural Logic Reinforcement Learning

Deep reinforcement learning (DRL) has achieved significant breakthroughs in various tasks. However, most DRL algorithms suffer a problem of generalizing the learned policy which makes the learning performance largely affected even by minor modifications of the training environment. Except that, the use of deep neural networks makes the learned policies hard to be interpretable. To address these two challenges, we propose a novel algorithm named Neural Logic Reinforcement Learning (NLRL) to represent the policies in reinforcement learning by first-order logic. NLRL is based on policy gradient methods and differentiable inductive logic programming that have demonstrated significant advantages in terms of interpretability and generalisability in supervised tasks. Extensive experiments conducted on cliff-walking and blocks manipulation tasks demonstrate that NLRL can induce interpretable policies achieving near-optimal performance while demonstrating good generalisability to environments of different initial states and problem sizes.

==> tex/arxiv.tex <==
\subsubsection{Tic-Tac-Toe}
We will then try a bit more complex task, tic-tac-toe, whose optimal policy is not so obvious.
In this experiment, we are first going to let the agent play against a random player.
Then we will try to use the self-play technique to train the agent.

Constants in this experiment are integers ${0,1,2}$.
The background knowledge in this task is again the basic knowledge about integers, which are \textit{zero(0)}, \textit{succ(0,1)} and \textit{succ(1,2)}.
The state is represented by three predicates, \textit{mine, opponent} and \textit{empty}, which specifies the ownership of each position on the board.
The action predicate is \textit{place(X,Y)}, which is valid only if the position $(X,Y)$ is empty. 
We will not prevent the agent from placing stones in invalid positions directly and let the agent learn it by itself.

==> tex/discussion.tex <==
\section{Discussion and Future Work} \label{sec:discussion}
Generalization towards larger problems is an attempting feature of NLRL.
Solving the problem by random moves will get less possible when the problems scale up, which can be observed by the performance of the random agents.
This also makes reinforcement learning agent hard to improve its policy by try and error.
Another type of generalization we did not try in our experiment is to transfer the predicates learned in easier tasks to more difficult ones.
We consider train the agent in a smaller or easier environment and generalize the policy to larger or harder problems will be a solution to sparse reward problems, deserving further research.

There are $p_A$ and $p_S$ in MDP with logic interpretation we proposed, which is hand-crafted in this work.
However, these might be replaced by neural networks in future, where replacing $p_A$ will be challenging but more important since in which case we can feed sensory data directly to the NLRL agent.

We observed that allow the agent to use more invented predicates than it really needs to express optimal policy will help the agent find the global optimal solution.
Such phenomenon coincides with neural networks, where more neurons in a layer help find global optima.
In recent years, the trend of neural networks is that larger networks can often solve more complex problems.
So an interesting question is if we scale the algorithm up, can we solve much more complex problems?
However, it is not easy to scale up the $\partial$ILP both in terms of the number of entities and the number of predicates.
On the other hand, there is neural theorem prover that scales up easier in terms of the number of entities and predicates but difficult to do deduction with more steps.
Therefore we consider improving the scalability of DILP algorithms as an important open question.

==> tex/dynamics.tex <==
\subsubsection{Learning Dynamics}
To demonstrate why the agent will be trapped in local minima, we consider a simple circumstance.
For target predicate $target()$, there are two definitions we care, $target(X) \leftarrow a1(X), a2(X)$ and $target(X) \leftarrow a1(X), pred(X)$, where $a1, a2$ are extensional predicates (either be state or background knowledge) and $pred$ is an invented predicate.
The two weights associated with these two clauses are, respectively, $w_{11}$ and $w_{12}$.
For $pred$ the useful definition is $pred(X) \leftarrow a2(X), a3(X)$ whose the weight associated is $w_{21}$.

The central task of policy gradient algorithms is to compute the $\frac{\partial V_{\pi}}{\partial \boldsymbol{w}}$, where $\pi$ is parametrised by $\boldsymbol{w}$ and $V_\pi$ is the value starting from the initial state following policy $\pi$.
Since $V_{\pi}$ is not differentialble, the estimation of it is used in practice, while we assume the estimation is precise here for sake of simplicity.
We denote the value of the sub-optimal policy $target(X) \leftarrow a1(X), a2(X)$ as $v1$,
the value of optimal policy $target(X) \leftarrow a1(X), a2(X), a3(X)$ as $v2$ and all other policies have the value of 0.
If the possibility of choosing an action is proportional to the valuations of that action atom, the possibility of following a policy is thus the product of weights related.
The value of the current policy $pi$ can then be expressed as
\begin{equation}
\begin{split}
V_\pi & = P(v_1|\boldsymbol{w}) v_1 + P(v_2|\boldsymbol{w}) v_2 \\
& = w_{11} v_1 + w_{21} w_{12} v_2
\end{split}
\end{equation}

Hence we can obtain the derivatives of the weights: 
$\frac{\partial V_{\pi}}{\partial w_{11}} = v_1$,
$\frac{\partial V_{\pi}}{\partial w_{12}} = v_2 w_{21}$,
$\frac{\partial V_{\pi}}{\partial w_{21}} = v_2 w_{12}$.

Suppose the initial weights of all the clauses are the same. 
If there are $m$ ($50<m<300$ in our experiments) possible clauses for each predicate, the direvative of both $w_{12}$ and $w_{21}$ will be $\frac{v_1}{m v_2}$ of the $w_{11}$.
Notably, since all the weights of a predicate sum up to 1, the $w_{11}$ and $w_{12}$ are competitive with each other (this constraint is added by softmax), which means the $w_{12}$ will decrease when all other weigths leads to 0 policy value is close to 0, and accordingly the increase step of $w_{12}$ will get smaller.
In Figure \ref{fig:discussion2}, we show the learning process when $m=100$ and $v_1, v_2$ takes different values.
Only when the value of optimal policy is significantly (60 times) larger than the suboptimal one, the $\partial ILP$ will converge to the global optima.
In practice, the situation may not be so bad as there can be some definitions of $pred$ that leads to other suboptimal policies which will not give 0 policy value.
However, it is easy to see that such problem will get more serious along with the increase of number of invented predicates involved and number of possible clauses.
\begin{figure}
\begin{subfigure}{.32\linewidth}
  \centering
  \includegraphics[width=\linewidth]{img/fig1.png}
  \caption{$v_1=1$, $v_2=2$}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
  \includegraphics[width=\linewidth]{img/fig2.png}
  \caption{$v_1=1$, $v_2=40$}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
  \centering
  \includegraphics[width=\linewidth]{img/fig3.png}
  \caption{$v_1=1$, $v_2=60$}
\end{subfigure}
\caption{Plots of the Learning Process}
\label{fig:discussion2}
\end{figure}

Although we merely analysed the $\partial$ILP trained with policy gradient here,
by replacing the $V_\pi$ as objective function, the same logic is likely to be apply on any gradient based optimization tasks.
In addition, other DILP algorithms such as NTP also share the similar problem mentioned here:
gradient related with multi-steps reasoning easily vanished because of the multiplications of the real number ranging from 0 to 1 (In NTP, such number is the proof score).
